Procurement and Purification of Liquid Argon for the LEGEND-200 Experiment

LEGEND-200 requires high-purity liquid argon for effective background discrimination. In this paper, we present the design, construction, and performance of a dedicated liquid argon purification system, along with the procurement and purification of liquid argon for filling the LEGEND-200 cryostat to its total capacity of 91 t. The purifier is based on copper catalyst and molecular sieve to remove oxygen and water. Starting with liquid argon of 5.5 quality, featuring an effective scintillation light triplet lifetime $\tau_t$ of about 0.9 $\mu$s, we achieved a final purity corresponding to $\tau_t$ = 1.3 $\mu$s. After complete filling of the LEGEND-200 cryostat, the measured effective triplet lifetime was 1.16 $\mu$s. The notable reduction is caused by a residual nitrogen impurity introduced by an accidentally spoiled liquid argon delivery. An excessive nitrogen influx was prevented by the LEGEND Liquid Argon Monitoring Apparatus (LLAMA), which served as one of the three independent purity monitors during the filling campaign.

==> definitions.tex <==
\RequirePackage{graphicx}
\usepackage{tikz}
\usepackage[separate-uncertainty=true, per-mode=symbol]{siunitx}
\usepackage{booktabs}
\usepackage{url} % or hyperref; we have at least one URL
\usepackage{hyperref}
\usepackage{multirow}
%\usepackage[numbers,unsrt]{natbib}
\usepackage[style=ieee]{biblatex}
\addbibresource{bibliography.bib}

\usepackage{amssymb}     % packages called in main file, e.g. gstr-template.tex
\usepackage{marvosym}    % symbols for EURO
\usepackage{upgreek}     % for upright greek letters in units
\usepackage{pgfplots, pgfplotstable}
\pgfplotsset{compat=1.14}
\let\note\relax % removes an error where \note is redefined by the callouts package in the next line
\usepackage[wby]{callouts}
\usepackage{siunitx}
\usepackage[version=4,arrows=pgf-filled]{mhchem}
\usepackage{hyperref}
\usepackage{ifthen}
\usepackage{orcidlink} % for ORCiD in authorlist, e.g. \orcidlink{0000-0002-8360-666X}


% units                  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\DeclareSIUnit[number-unit-product = {}]{\inchQ}{\ensuremath{{}^{\prime\prime}}}
\DeclareSIUnit[number-unit-product = {\thinspace}]{\inch}{in}
\DeclareSIUnit\year{yr}  
\DeclareSIUnit\ckky{cts/(keV \; kg \; yr)}  
\DeclareSIUnit\angstrom{\text{Å}}
\DeclareSIUnit\bar{bar}

\newcommand{\beq} {\begin{equation}}
\newcommand{\eeq} {\end{equation}}


\newcommand{\versionabb}  {version 10.4 dated 20140902}
%
\newcommand{\ctsa}        {cts/(d$\times$m$^2$)}
\newcommand{\ctsper}      {cts/(keV$\times$kg$\times$yr)}
%\newcommand{\ctsper}      {cts/(keV$\cdot$kg$\cdot$yr)}
\newcommand{\ctsperee}    {cts/(keV$_{ee}\cdot$kg$\cdot$yr)}
\newcommand{\ctsperrec}   {cts/(keV$_{rec}\cdot$kg$\cdot$yr)}
\newcommand{\zctsper}     {{$10^{-2}$~cts/(keV$\cdot$kg$\cdot$yr)}}
\newcommand{\tctsper}     {{$10^{-2}$~cts/(keV$\cdot$kg$\cdot$yr)}}
\newcommand{\pIbi}        {{$10^{-2}$~cts/(keV$\cdot$kg$\cdot$yr)}}
\newcommand{\dctsper}     {{$10^{-3}$~cts/(keV$\cdot$kg$\cdot$yr)}}
\newcommand{\pIIbi}       {{$10^{-3}$~cts/(keV$\cdot$kg$\cdot$yr)}}
\newcommand{\biperton}    {{1~cts/(keV$\cdot$t$\cdot$yr)}}
\newcommand{\vctsper}     {{$10^{-4}$~cts/(keV$\cdot$kg$\cdot$yr)}}
\newcommand{\ctsperx}     {$\frac{10^{-3}\rm cts}{\rm keV\cdot kg \cdot yr}$}
\newcommand{\kgy}         {{kg$\cdot$yr}}
\newcommand{\kgyr}        {{kg$\cdot$yr}}
\newcommand{\kevkgyr}     {{keV$\cdot$kg$\cdot$yr}}
\newcommand{\cum}         {{m$^3$}}
\newcommand{\mubq}        {{$\upmu$Bq}}
\newcommand{\mum}         {{$\upmu$m}}
\newcommand{\mus}         {{$\upmu$s}}
%\newcommand{\mubqperkg}   {{$\frac{\upmu\mathrm{Bq}}{\mathrm{kg}}$}}
\newcommand{\mubqperkg}   {{${\upmu\mathrm{Bq}}/{\mathrm{kg}}$}}
%
\def\cpowten#1#2{{$#1\cdot10^{#2}$}}
\def\powten#1{{$10^{#1}$}}
%
\newcommand{\C}           {$^\circ$C}
\newcommand{\al}          {$\alpha$}
\newcommand{\be}          {$\beta$}
\newcommand{\ga}          {$\gamma$}
\newcommand{\gam}         {$\gamma$}
\newcommand{\gammas}      {$\gamma${s}}
\newcommand{\qbb}         {{$Q_{\beta\beta}$}}
\newcommand{\thalf}       {${T_{1/2}}$}
\newcommand{\thalfzero}   {${T^{0\nu}_{1/2}}$}
\newcommand{\thalftwo}    {${T^{2\nu}_{1/2}}$}
\newcommand{\nmez}        {${\cal M}^{0\nu}$}
\newcommand{\nmet}        {${\cal M}^{2\nu}$}
% dbd                     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bb}          {{$\beta\beta$}}
\newcommand{\bbno}        {{$0\nu\beta\beta$}}
\newcommand{\onbb}        {{$0\nu\beta\beta$}}
\newcommand{\nnbb}        {{$2\nu\beta\beta$}}
\newcommand{\twonu}       {{$2\nu\beta\beta$}}
% other usefull           %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tlive}       {\mbox{$t_{live}$}}
\newcommand{\flive}       {\mbox{$f_{live}$}}
\newcommand{\fge}         {\mbox{$f_{Ge}$}}
\newcommand{\fgesix}      {\mbox{$f_{76}$}}
\newcommand{\fgesixi}     {\mbox{$f_{76,i}$}}
\newcommand{\actmass}     {\mbox{$M_{act}$}}
\newcommand{\ssmass}      {\mbox{$M_{76}$}}
\newcommand{\factmass}    {\mbox{$f_{av}$}}
\newcommand{\factmassi}   {\mbox{$f_{av,i}$}}
\newcommand{\factvol}     {\mbox{$f_{av}$}}
\newcommand{\factvoli}    {\mbox{$f_{av,i}$}}
\newcommand{\subssix}     {\mbox{$_{76}$}}
\newcommand{\subssixi}    {\mbox{$_{76,i}$}}
\newcommand{\subav}       {\mbox{$_{av}$}}
\newcommand{\subavi}      {\mbox{$_{av,i}$}}
%\newcommand{\ }
%% spacings for tables etc %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bal}         {\rule{10mm}{0.2mm}}
\newcommand{\balf}        {\rule{10mm}{2mm}}
\newcommand{\tabta}       {\rule[-1,5mm]{0mm}{7,5mm}}
\newcommand{\tabtag}      {\rule[-3mm]{0mm}{9mm}}
\newcommand{\up}          {\rule{0mm}{5mm}}
\newcommand{\down}        {\rule[-2mm]{0mm}{3mm}}
% for literature
\newcommand{\etal}        {\textit{et al.}}
\newcommand{\bulitem}     {\item[{\large$\bullet$}]}
\newcommand{\prep}        {\textit{Preprint}}
\newcommand{\NIM}         {Nucl.~Instr.~Meth.}
\newcommand{\PRB}         {Phys.~Rev.~B}
\newcommand{\mpik}        {\mbox{MPI-K}}
\newcommand{\mpip}        {\mbox{MPI-P}}
% experiments and equipment  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\gerda}       {\textsc{Gerda}}
\newcommand{\G}           {{\mbox{\textsc{Gerda}}}}
\newcommand{\gd}          {\mbox{\textsc{Gerda}}}  
%
\newcommand{\lngs}        {{\mbox{\textsc{Lngs}}}}
\newcommand{\LNGS}        {{\mbox{\textsc{Lngs}}}}
\newcommand{\WT}          {water tank}
\newcommand{\lar}         {LAr}
\newcommand{\geni}        {{\mbox{\textsc{Genius}}}}
\newcommand{\gdl}         {\textsc{Gdl}}
\newcommand{\gerdalarge}  {\textsc{Gerda-LArGe}}
\newcommand{\bege}        {{\sc BEGe}}
\newcommand{\phaseone}    {Phase~I}
\newcommand{\phasetwo}    {Phase~II}
\newcommand{\phasetwop}   {Phase~II$^+$}

\newcommand{\morex}       {\textsc{MoREx}}
\newcommand{\morexino}    {\textsc{MoRExino}}
\newcommand{\LArGe}       {\textsc{LArGe}}
\newcommand{\largee}      {\textsc{LArGe}}
\newcommand{\SUB}         {{\mbox{\text{SUB}}}}
\newcommand{\Gerdella}    {{\mbox{\textsc{Gerdella}}}}
\newcommand{\GeMPI}       {Ge\textsc{MPI}}
\newcommand{\GEMPI}       {Ge\textsc{mpi}}
%    other exps.          %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\majorana}    {\textsc{Majorana}}
\newcommand{\Majorana}    {{\mbox{\textsc{Majorana}}}}
\newcommand{\MAJORANA}    {{\sc Majorana}}
\newcommand{\eureca}      {{\sc Eureca}}
\newcommand{\igex}        {\textsc{Igex}}
\newcommand{\legend}      {\textsc{Legend}}
\newcommand{\scarf}      {\textsc{Scarf}}
\newcommand{\IGEX}        {{\mbox{\textsc{Igex}}}}
\newcommand{\hdm}         {\textsc{HdM}}
\newcommand{\HdM}         {\mbox{\textsc{HdM}}}  
\newcommand{\HDM}         {\mbox{\textsc{HdM}}}  
\newcommand{\BX}          {\mbox{\textsc{Borexino}}}
\newcommand{\borex}       {\mbox{\textsc{Borexino}}}
\newcommand{\borexino}    {\mbox{\textsc{Borexino}}}
\newcommand{\EUROBALL}    {\textsc{Euroball}}
\newcommand{\ICARUS}      {\textsc{Icarus}}
\newcommand{\LENS}        {\textsc{Lens}}
\newcommand{\STRAW}       {\textsc{Straw}}
\newcommand{\Gallex}      {\textsc{Gallex}}
\newcommand{\Sage}        {\textsc{Sage}}
\newcommand{\LVD}         {{\mbox{\textsc{Lvd}}}}
\newcommand{\GNO}         {{\mbox{\textsc{Gno}}}}
\newcommand{\KAMLAND}     {{\mbox{\textsc{KAMland}}}}
\newcommand{\CUORI}       {{\mbox{\textsc{Cuoricino}}}}
\newcommand{\CUORE}       {{\mbox{\textsc{Cuore}}}}
\newcommand{\cuore}       {{\mbox{\textsc{Cuore}}}}
\newcommand{\AGATA}       {{\mbox{\textsc{Agata}}}}
\newcommand{\WMAP}        {{\mbox{\textsc{Wmap}}}}
\newcommand{\NEMO}        {{\mbox{\textsc{Nemo}}}}
\newcommand{\KATRIN}      {{\mbox{\textsc{Katrin}}}}
\newcommand{\MOON}        {{\mbox{\textsc{Moon}}}}
\newcommand{\EXO}         {{\mbox{\textsc{Exo}}}}
\newcommand{\GEM}         {{\mbox{\textsc{Gem}}}}
\newcommand{\CAMEO}       {{\mbox{\textsc{Cameo}}}}
\newcommand{\COBRA}       {{\mbox{\textsc{Cobra}}}}
\newcommand{\CRYOGENM}    {{\mbox{\textsc{Cryogenmash}}}}
\newcommand{\xenon}       {{\mbox{\textsc{Xenon}}}}
\newcommand{\Xenon}       {{\mbox{\textsc{Xenon}}}}
\newcommand{\taiga}       {{\mbox{\textsc{Taiga}}}}
\newcommand{\nxt}         {{\mbox{\textsc{NEXT}}}}
\newcommand{\ds}          {{\mbox{\textsc{Dark}\textsc{Side}}}}
\newcommand{\dss}          {DS}
\newcommand{\sk}          {Super-Kamiokande}
\newcommand{\kam}         {Kamiokande}
\newcommand{\kzen}        {KamLAND-Zen}
\newcommand{\kamland}     {KamLAND}
\newcommand{\sno}         {{\mbox{\textsc{SNO+}}}}
\newcommand{\snemo}       {SuperNEMO}
\newcommand{\cd}         {{\mbox{\textsc{Candless}}}}

% codes                   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\geant}       {\textsc{Geant4}}
\newcommand{\GEANT}       {\textsc{\mbox{{Geant}}}}
\newcommand{\rootv}       {\textsc{Root}}
\newcommand{\CERN}        {{\mbox{\textsc{Cern}}}}
\newcommand{\mage}        {\textsc{MaGe}}
\newcommand{\gelatio}     {\textsc{Gelatio}}
\newcommand{\mgdo}        {\mbox{MGDO}}
\newcommand{\tier}        {\textsc{Tier}}
\newcommand{\psa}         {Pulse Shape Analysis}
% isotopes                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\gesix}       {{$^{76}$Ge}}
\newcommand{\geseven}     {{$^{77}$Ge}}
\newcommand{\gefour}      {{$^{74}$Ge}}
\newcommand{\gethree}     {{$^{73}$Ge}}
\newcommand{\gess}        {{$^{76}$Ge}}
\newcommand{\gesf}        {{$^{74}$Ge}}
\newcommand{\geenr}       {{$^{\rm enr}$Ge}}          %$^{\rm enr}$Ge
\newcommand{\genat}       {{$^{\rm nat}$Ge}}
\newcommand{\gedep}       {{$^{\rm dep}$Ge}}
\newcommand{\geox}        {{GeO$_2$}}
\newcommand{\enrgecoax}   {{$^{\rm enr}$Ge-coax}} 
\newcommand{\nuc}[2]      {{$^{#2}\rm #1$}}
\newcommand{\cosix}       {{$^{60}$Co}}
\newcommand{\radzzs}      {{$^{226}$Ra}}
\newcommand{\thzza}       {{$^{228}$Th}}
\newcommand{\tlzna}       {{$^{208}$Tl}}
\newcommand{\kvn}         {{$^{40}$K}}
\newcommand{\kvz}         {{$^{42}$K}}
\newcommand{\Am}          {$^{241}$Am}
\newcommand{\Ra}          {$^{226}$Ra}
\newcommand{\Po}          {$^{210}$Po}
\newcommand{\Ar}          {$^{39}$Ar}
\newcommand{\arr}         {$^{42}$Ar}
\newcommand{\krr}         {$^{42}$K}
\newcommand{\Kr}          {$^{85}$Kr}
\newcommand{\ar}          {$^{39}$Ar}
\newcommand{\kr}          {$^{85}$Kr}
\newcommand{\Xe}          {$^{133}$Xe}
\newcommand{\Ba}          {$^{133}$Ba}
\newcommand{\Bi}          {$^{214}$Bi}
\newcommand{\Biz}         {$^{210}$Bi}
\newcommand{\bi}          {$^{210}$Bi}
\newcommand{\Yb}          {$^{176}$Yb}
\newcommand{\Fe}          {$^{55}$Fe}
\newcommand{\Th}          {$^{228}$Th}
\newcommand{\Thh}         {$^{232}$Th}
\newcommand{\Tl}          {$^{208}$Tl}
\newcommand{\Ul}          {$^{235}$U}
\newcommand{\Uh}          {$^{238}$U}
\newcommand{\Be}          {$^7$Be}
\newcommand{\YO}          {Yb$_2$O$_3$}
\newcommand{\Co}          {$^{60}$Co}
\newcommand{\Rnd}         {$^\mathsf{222}$Rn}
\newcommand{\Rnz}         {$^{220}$Rn}
\newcommand{\Pb}          {$^{210}$Pb}
\newcommand{\Poo}         {$^{218}$Po}
\newcommand{\Poc}         {$^{214}$Po}

\newcommand{\nit}         {N$_2$}
\newcommand{\oxy}         {O$_2$}
\newcommand{\water}       {H$_2$O}
\newcommand{\llars}       {LLArS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\exposure}    {\mbox{$\cal E$}}
\newcommand{\effqual}     {\mbox{$\varepsilon_{qcut}$}}
\newcommand{\effpsd}      {\mbox{$\varepsilon_{psd}$}}
\newcommand{\effres}      {\mbox{$\varepsilon_{res}$}}
\newcommand{\efffep}      {\mbox{$\varepsilon_{fep}$}}
\newcommand{\effquali}     {\mbox{$\varepsilon_{qcut,i}$}}
\newcommand{\effpsdi}      {\mbox{$\varepsilon_{psd,i}$}}
\newcommand{\effresi}      {\mbox{$\varepsilon_{res,i}$}}
\newcommand{\efffepi}      {\mbox{$\varepsilon_{fep,i}$}}
%
\newcommand{\effmuon}     {\mbox{$\varepsilon_\mu$}}
\newcommand{\effmurej}    {\mbox{$\varepsilon_{rej}$}}
\newcommand{\effmureji}    {\mbox{$\varepsilon_{rej,i}$}}
\newcommand{\coll}         {Collaboration}
\newcommand{\carboact}     {CarboAct\textsuperscript{\textregistered}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%new
\newcommand{\llama}{LLA\-MA}
